Theoretical Models of Learning to Learn

A Machine can only learn if it is biased in some way. Typically the bias is supplied by hand, for example through the choice of an appropriate set of features. However, if the learning machine is embedded within an {\em environment} of related tasks, then it can {\em learn} its own bias by learning sufficiently many tasks from the environment. In this paper two models of bias learning (or equivalently, learning to learn) are introduced and the main theoretical results presented. The first model is a PAC-type model based on empirical process theory, while the second is a hierarchical Bayes model.

==> mathdefs.tex <==
\newcommand{\supp}{{\mbox{supp}}}
\newcommand{\bb}{\mathbb}
\renewcommand{\Box}{\qed}
\newcommand{\mathbold}[1]{\mbox{\boldmath $\bf#1$}}
\newcommand{\glossaryentry}[3]{\item[#1] #2 \hfill #3}
\renewcommand{\glossary}[2]{}
\def\addcontentsline#1#2#3{} 
\renewcommand{\thickapprox}{\doteq}
\newtheorem{thm}{Theorem}
\newtheorem{exmp}{Example}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{corr}[thm]{Corollary}
\newtheorem{defn}{Definition}
\newcommand{\D}{{\cal D}}
\DeclareMathOperator{\er}{er}
\DeclareMathOperator{\VCdim}{VCdim}
\newcommand{\erh}{{\hat{\er}}}
\newcommand{\ie}{{\em i.e.\ }}
\newcommand{\etal}{{\em et.\ al.\ }}
\newcommand{\iid}{{i.i.d.\ }}
\newcommand{\norm}{{\|\cdot\|}}
\newcommand{\eg}{{\em e.g.\ }}
\newcommand{\cf}{{\em c.f.\ }}
\newcommand{\etc}{{\em etc\ }}
\newcommand{\comp}[2]{{#1\circ#2}}
\newcommand{\epspic}[2]{{\parbox{#1}{\epsfxsize=#1\epsfbox{#2}}}}
\renewcommand{\d}[2]{d_\nu\left(#1,#2\right)}
\newcommand{\pt}{p(z|\theta)}
\newcommand{\ptt}{p(z|\thetat)}
\newcommand{\rangel}[1]{\rangle_{#1}}
\newcommand{\E}{\bb E}
\newcommand{\HH}{{\bb H}}
\newcommand{\Hs}{{\HH_\sigma}}
\renewcommand{\H}{{\cal H}}
\newcommand{\XY}{{X\times Y}}
\newcommand{\VY}{{V\times Y}}
\newcommand{\de}{=}%%{{\,\,\,\,\overset{\text{def}}{=}\,\,\,\,}}
\renewcommand{\P}{{\cal P}}
\newcommand{\Zm}{{Z^m}}
\newcommand{\Zn}{{Z^n}}
\newcommand{\Zmn}{{Z^{(m,n)}}}
\newcommand{\Znm}{{Z^{(n,m)}}}
\newcommand{\Ztmn}{{Z^{(2m,n)}}}
\newcommand{\Gtmn}{{\Gamma_{(2m,n)}}}
\newcommand{\zmn}{{z^{(m,n)}}}
\newcommand{\znm}{{z^{(n,m)}}}
\newcommand{\znmm}{{z^{(n,m-1)}}}
\newcommand{\z}{{\mathbold{z}}}
\newcommand{\f}{{\bf f}}
\newcommand{\g}{{\bf g}}
\newcommand{\w}{{\bf w}}
\newcommand{\x}{{\bf x}}
\newcommand{\y}{{\bf y}}
\newcommand{\B}{{\cal B}}
\newcommand{\h}{{\mathbold{h}}}
\newcommand{\Q}{{\cal Q}}
\newcommand{\Pm}{{P^m}}
\newcommand{\zb}{{\bold{z}}}
\newcommand{\zbh}{{\hat{\zb}}}
\newcommand{\zbv}{{\smash[b]{\vec{\zb}}}}
\newcommand{\zbvh}{\zbv} %%{\smash[b]{\hat{\vec{\zb}}}}}
\newcommand{\zh}{{\hat z}}
\newcommand{\xh}{{\hat x}}
\newcommand{\sh}{{\hat s}}
\newcommand{\Xhat}{{\hat X}}
\newcommand{\Shat}{{\hat S}}
\newcommand{\Ehat}{{\hat E}}
\newcommand{\qhat}{{\hat q}}
\newcommand{\yh}{{\hat y}}
\newcommand{\Phat}{{\hat \P}}
\newcommand{\Ph}{{\hat P}}
\newcommand{\zs}{{\z_\sigma}}
\newcommand{\zsw}{{\z_\sigma(1)}}
\newcommand{\zst}{{\z_\sigma(2)}}
\newcommand{\zsij}{{\z_{\sigma(ij)}}}
\newcommand{\fhat}{{\hat f}}
\newcommand{\ghat}{{\hat g}}
\newcommand{\Fhat}{{\hat \F}}
\newcommand{\rhat}{{\hat \rho}}
\newcommand{\Eh}{{\hat E}}
\newcommand{\bw}{{\bold{w}}}
\newcommand{\be}{\begin{equation*}}
\newcommand{\ee}{$$}
\newcommand{\ep}{{\varepsilon}}
\newcommand{\Z}{{\cal Z}}
\newcommand{\A}{{\cal A}}
\newcommand{\C}{{\cal C}}
\newcommand{\N}{{\cal N}}
\newcommand{\Nco}{{\N_\co}}
\newcommand{\M}{{\cal M}}
\newcommand{\F}{{\cal F}}
\newcommand{\G}{{\cal G}}
\newcommand{\T}{{\bb T}}
\newcommand{\U}{{\cal U}}
\newcommand{\V}{{\cal V}}
\renewcommand{\S}{{\cal S}}
\newcommand{\Ch}{{\hat \C}}
\newcommand{\rhol}{\rho_{\!_l}}
\renewcommand{\(}{\left(}
\renewcommand{\)}{\right)}
\renewcommand{\[}{\left[}
\renewcommand{\]}{\right]}
\newcommand{\Pv}{{\vec{P}}}
\newcommand{\xb}{{\bold{x}}}
\newcommand{\yb}{{\bold{y}}}
\newcommand{\wb}{{\bold{w}}}
\newcommand{\Fbar}{{\overline\F}}
\newcommand{\Rbar}{{\overline R}}
\newcommand{\Cbar}{{\overline C}}
\newcommand{\Lbar}{{\overline L}}
\newcommand{\Gbar}{{\overline\G}}
\newcommand{\Pbar}{{\bar{P}}}
\newcommand{\Pb}{{\mathbold{P}}}
\newcommand{\scPb}{{\mathbold{\scriptstyle P}}}
\renewcommand{\hbar}{{\overline h}}
\newcommand{\dbar}{{d^*}}
\newcommand{\co}{{\text{\rm co}}}
\newcommand{\jon}{{\text{\rm jon}}}
\newcommand{\cdm}{{d_{\text{\rm CDM}}}}
\newcommand{\cdmhat}{{\hat{d}_{\text{\rm CDM}}}}
\newcommand{\thetahat}{{\hat{\theta}}}
\newcommand{\pihat}{{\hat{\pi}}}
\newcommand{\thetat}{{\tilde{\theta}}}
\newcommand{\cdmhathat}{{\tilde{d}_{\text{\rm CDM}}}}
\newcommand{\lin}{{\text{\rm lin}}}
\newcommand{\sign}{{\text{\rm sign}}}
\newcommand{\IID}{{\text{\rm IID}}}
\newcommand{\OTS}{{\text{\rm OTS}}}
\newcommand{\CDM}{{\text{\rm CDM}}}
\newcommand{\VC}{{\text{\rm VC}}}
\newcommand{\LDR}{{\text{\rm LDR}}}
\newcommand{\OUT}{{\text{\rm OUT}}}
\newcommand{\cobar}[1]{{\overline{\text{\rm co}\(#1\)}}}
\newcommand{\linbar}[1]{{\overline{\text{\rm lin}\(#1\)}}}
\newcommand{\fbar}{{\bar f}}
\newcommand{\lbar}{{\bar l}}
\newcommand{\pibar}{{\bar \pi}}
\newcommand{\zv}{{\vec{z}}}
\newcommand{\gv}{{\vec{g}}}
\newcommand{\fv}{{\vec f}}
\newcommand{\lv}{{\vec l}}
\newcommand{\hv}{{\vec h}}
\newcommand{\xv}{{\vec x}}
\newcommand{\yv}{{\vec y}}
\newcommand{\wv}{{\vec w}}
\newcommand{\vv}{{\vec v}}
\newcommand{\av}{{\vec a}}
\newcommand{\Xv}{{\vec X}}
\newcommand{\pr}[3]{{{#1}_1#2\dots#2{#1}_{#3}}}
\newcommand{\iton}{{1\leq i\leq n}}
\newcommand{\prd}[4]{{{#1}_{#2}#3\dots#3{#1}_{#4}}}
\newcommand{\R}{{\mathbb R}}
\newcommand{\Rn}{{\R^n}}
\newcommand{\Rpm}{{(\bb R^+)^{2m}}}
\newcommand{\Rptm}{{(\bb R^+)^{(2m,n)}}}
\newcommand{\dl}{{\mbox{\boldmath$d_{L^1}$}}}
\newcommand{\dimp}{{\mbox{dimp}}}
\newcommand{\argmin}{{\mbox{argmin}}}
\newcommand{\plus}{{\mbox{plus}}}
\newcommand{\minus}{{\mbox{minus}}}
\newcommand{\DKL}{{\mbox{DKL}}}
\newcommand{\WKS}{{\mbox{WKS}}}
\newcommand{\PKS}{{\mbox{PKS}}}
\newcommand{\ch}{{\large \chi}}
\newcommand{\SZ}{{\cal S}_Z}
\newcommand{\SP}{{\cal S}_\P}
\newcommand{\Tbar}{{\overline T}}
\newcommand{\Sbar}{{\overline S}}
\newcommand{\Xbar}{{\overline X}}
\newcommand{\Hbar}{{\overline \H}}
\newcommand{\bool}{{\{\pm 1\}}}
\newcommand{\zm}{{z^m}}
\newcommand{\Hns}{{\[\HH^n\]_\sigma}}
\newcommand{\Hsn}{{\[\HH_\sigma\]^n}}
\newcommand{\XVA}{X\stackrel{\F}{\rightarrow}V\stackrel{\G}{\rightarrow}A}
\newcommand{\XfVGY}{X\stackrel{f}{\rightarrow}V\stackrel{\G}{\rightarrow}Y}










